Autoformalization with Large Language Models

Autoformalization is the process of automatically translating from natural language mathematics to formal specifications and proofs. A successful autoformalization system could advance the fields of formal verification, program synthesis, and artificial intelligence. While the long-term goal of autoformalization seemed elusive for a long time, we show large language models provide new prospects towards this goal. We make the surprising observation that LLMs can correctly translate a significant portion ($25.3\%$) of mathematical competition problems perfectly to formal specifications in Isabelle/HOL. We demonstrate the usefulness of this process by improving a previously introduced neural theorem prover via training on these autoformalized theorems. Our methodology results in a new state-of-the-art result on the MiniF2F theorem proving benchmark, improving the proof rate from $29.6\%$ to $35.2\%$.

==> sections/checklist.tex <==
\newpage
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See discussion section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See discussion section.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{It is expensive to run multiple times, and we believe the results are significant.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{sec:ntp}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}{We cited the creators of the assets when we first mentioned them.}
  \item Did you mention the license of the assets?
    \answerYes{We included the links to the licenses of the assets when we first mentioned them in Section~\ref{sec: exp}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include the code we used to train the models in the supplemental material. The data we used are all under open-source licenses.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{The assets we used mostly have open-sourced licenses as mentioned previously.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{The data we used are mathematical proofs so we think it is apparent that they do not contain personally identifiable information or any offensive content.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> sections/conclusion.tex <==
% \section{Discussion}

% We demonstrate, for the first time, that 

% Comparison to the recent OAI result:
% - MiniF2F result relies human translator; expensive data. We automate that, get more data.
% - IMO result relies on specific synthetic data.




==> sections/intro_backup.tex <==
\section{Introduction}

% History
% Challenge: disconnect from human mathematics,
% Recent advances in ML allow us to work directly with natural language texts.

% Mathematical reasoning has been a central goal of artificial intelligence since its early days~\citep{mccarthy1961computer}, and today there are a number of fields devoted to these ideas, including interactive theorem provers, computer algebra systems, verification, and arguably many more.
% While each of these fields have impressive applications, the ambition to automate mathematics has been elusive.
%
Automation in theorem proving has made significant advances by the inroads of \emph{neural theorem provers} ~\citep{huang2018gamepad,bansal2019holist,polu2020gptf,wu2021tacticzero}, which use neural networks to predict proofs that can be checked by interactive theorem provers.
However, the lack of training data in the form of formally specified statements and definitions has been a limiting factor, as only a minor fraction of mathematics has been formalized and most of mathematics is available exclusively in natural language.
% Our quest for autoformalization is motivated by our need of tapping into the vast amount of natural language mathematics that could enable us to train strong, automated neural reasoning engines with correctness guarantees that rival or exceed human performance. % This would be  were we able to translate a significant portion of the existing human mathematics into formally verifiable format and train neural theorem provers on them.
% While this long-term goal is still elusive, we present a first proof of concept for this idea using the Isabelle proof assistant, the MiniF2F benchmark~\citep{zheng2021minif2f} and the capabilities of the latest large language models like Codex~\citep{chen2021codex} and PaLM~\citep{chowdhery2022palm}, that were trained on a large amount of web data in a self-supervised manner.

% % Since the dawn of AI research, symbolic logic has promised the ability for machines to reason, up to and including AGI. It has fallen drastically short of this promise. Current efforts in this direction are limited by the dearth of data: there just is not that much meaningful text written in symbolic logic, at least compared to other areas. In this paper, we show how modern large language models may be used to translate some of the vast quantity of mathematics written by humans for humans into symbolic logic. These translations are not reliable, but enough of them are correct to produce significant additional training data. As proof of principle, we use this synthetically generated and verified training data to improve upon the SoTA for the miniF2F theorem proving benchmark. While this paper is only an early step in this direction, we expect that reasoning engines trained in lockstep with autoformalizers may end up rivaling the performance of human mathematicians in the not too far future.

% Mathematical reasoning has been a central goal of artificial intelligence since its early days~\citep{mccarthy1961computer}, and today there are a number of fields devoted to these ideas, including computer algebra systems, automated theorem proving, verification, interactive theorem assistants and arguably many more.
% While each of these fields have impressive applications, they are disconnected from the largest body of mathematical knowledge: the books and articles written by mathematicians.
% Hence, their methods rely on human experts to encode problems appropriately and often get stuck on problems that would be easy to solve for human mathematicians.

% A few important and complex results of mathematics and computer science have been formalized manually using \emph{interactive theorem provers}, such as the four color theorem~\citep{gonthier2008formal}, the Kepler conjecture~\citep{hales2017formal}, the odd-order theorem~\citep{gonthier2013odd} and the verification of a microkernel~\citep{Klein2009seL4}. Interactive theorem provers, such as Isabelle~\citep{wenzel08isabelle}, \cite{coq}, HOL Light~\citep{Harrison96hollight}, and Lean~\citep{demoura2015lean} are programming languages that enable users to enter their definitions, statements and proofs in a formal language, which can then be checked automatically for correctness.
% % Several important results of mathematics and computer science have been formalized in interactive theorem provers, such as the four color theorem~\citep{gonthier2008formal}, the Kepler conjecture~\citep{hales2017formal}, and the verification of a microkernel~\citep{Klein2009seL4}.
% % While these projects helped to gain a very high level of certainty about the correctness of their results, they were also extremely labor intensive.
% Recently, the long-standing goal of automating proof search has made a lot of progress with the advent of proof automation to predict proof steps in interactive theorem provers ~\citep{GauthierKUKN21TacTicToe}.  Around the same time, several \emph{neural theorem provers} were introduced for various proof assistants 
% %(Coq, HOL-Light, Metamath, Isabelle and Lean)
% ~\citep{GauthierKUKN21TacTicToe,huang2018gamepad,bansal2019holist,polu2020gptf,wu2021tacticzero,han2022pact}.
% One of the main challenges with neural theorem provers is the scarcity of training data, while modern neural learning systems require vast amounts of them for strong results.
% The ability to use natural language mathematics as an additional source of data would hence help tremendously.

\emph{Autoformalization} refers to the task of automatically translating from natural language mathematics to a formal language, such as an interactive theorem prover~\citep{szegedy2020promisingpath}.
While this long-term goal seemed elusive for a long time,
recent advances in machine learning for natural language make autoformalization appear more and more realistic.
The most recent generation of large language models has not only impressive capabilities to process text, but also show significant improvements at solving school-level mathematical text problems~\citep{chowdhery2022palm}. 
Codex \citep{chen2021codex} and Alphacode \citep{Li2022alphacode} have further shown that large language models can already write small programs given natural language instructions, which raises the question whether large language models are suitable for autoformalization.

In this work, we demonstrate that autoformalization is helpful for the training of neural theorem provers.
First, we make the surprising observation that large language models already have a decent capability of formalizing natural language mathematics in an interactive theorem prover.
We present several automatically generated formalizations (and informalizations) in case studies and classify the typical failure modes in an analysis of 150 randomly picked formalizations.
While only some portion of these formalizations would be considered correct, we demonstrate that autoformalization can provide useful training data for neural theorem provers.
We use autoformalized statements as targets for proof search with a neural theorem prover for Isabelle/HOL.
After fine-tuning our neural theorem prover on the proofs it found, its success rate on the MiniF2F benchmark~\citep{zheng2021minif2f} increases significantly, achieving a new state-of-the-art result of 35.2\% theorems proven.

